Leveraging Decision Diagrams to Solve Two-stage Stochastic Programs with Binary Recourse and Logical Linking Constraints

Two-stage stochastic programs with binary recourse are challenging to solve and efficient solution methods for such problems have been limited. In this work, we generalize an existing binary decision diagram-based (BDD-based) approach of Lozano and Smith (Math. Program., 2018) to solve a special class of two-stage stochastic programs with binary recourse. In this setting, the first-stage decisions impact the second-stage constraints. Our modified problem extends the second-stage problem to a more general setting where logical expressions of the first-stage solutions enforce constraints in the second stage. We also propose a complementary problem and solution method which can be used for many of the same applications. In the complementary problem we have second-stage costs impacted by expressions of the first-stage decisions. In both settings, we convexify the second-stage problems using BDDs and parametrize either the arc costs or capacities of these BDDs with first-stage solutions depending on the problem. We further extend this work by incorporating conditional value-at-risk and we propose, to our knowledge, the first decomposition method for two-stage stochastic programs with binary recourse and a risk measure. We apply these methods to a novel stochastic dominating set problem and present numerical results to demonstrate the effectiveness of the proposed methods.

==> benders_cuts.tex <==
\section{Cut Derivation for Benders Algorithm} \label{sec:benders}

In this section, we will describe how to derive cuts for $\Primal{3}{1}$ and explain how to strengthen the cuts derived from both BDD-based methods.



	
\subsection{BDD-based Benders Cuts} \label{subsec:bddbenderscuts}

For a fixed scenario $\omega$ the Benders cuts that come from \bdd{2} are:

 \begin{equation}  \label{eq:bdd1_cuts}
 \eta_\omega \geq \hat{\pi}_\rootnode - \sum_{a  \in \arcs^\omega} \sum_{i \in \viol_a} \hat{\beta}_{aq}(1 - \indvar_i).
\end{equation} 

For a scenario BDD $\BDD^\omega$ and master problem solution $\hat{\indvar}$ we calculate the dual solutions using a bottom-up shortest-path algorithm, as described in \cite{lozano2018bdd}. The terminal has dual value $\pi_\term = 0$ and each subsequent BDD node $i$ has dual value $\pi_i$, the length of the shortest path from $i$ to $\term$. The $\beta_{aq}$ variables are only on those arcs with capacities, for such an arc $a = (i,j)$ if $\pi_i - \pi_j$ is shorter than the arc length, that is the shortest path does not lie on $a$, then $\beta_{aq} = 0$ for all $q \in \viol_a$. Otherwise,  if $a \in \zeroarcs$ we have $\pi_i - \pi_j > 0$, so for  some arbitrary $\bar{q} \in \viol_a$ where $\mpsol^\omega_q = 1$ we set $\beta_{a\bar{q}} = \pi_i - \pi_j $ and $\beta_{aq} = 0$ for all $q \neq \bar{q} \in \viol_a$. Similarly, if $a \in \onearcs$ we have $\pi_i - \pi_j - \yweights_{\map(a)}> 0$, then we set $\beta_{a\bar{q}} = \pi_i - \pi_j -  \yweights_{\map(a)}$ for an arbitrary $\bar{q} \in \viol_a$ where $\mpsol^\omega_q = 1$, and set and $\beta_{aq} = 0$ for all $q \neq \bar{q} \in \viol_a$. These dual values can be computed in linear time with respect to the number of arcs in the BDD.


 \begin{example} \label{ex:bdd1_cuts}
 	
 Recall, in Example \ref{ex:bdd1}, we built the BDD for the scenario graph in Figure \ref{fig:smwds_graph}, we will now use this BDD to compute a cut for a master problem solution $\hat{\xvar} = [0,0,1,0,0]$. This solution has $\xvar_2 = 1$, thus any arc where $\xvar_2$ appears in all the capacity expressions will not be interdicted. 
 In Figure \ref{fig:bdd1_cuts} those arcs which still have capacity $0$ are highlighted. We are then able to compute the dual values $\pi$ using the bottom up shortest path algorithm and obtain $\pi_\rootnode =1$. The dual values of each node are given inside the node in Figure \ref{fig:bdd1_cuts}. 
 Finally, to derive the cut we must compute the 
 values of $\beta_{aq}$. We observe that to have $\beta_{aq} \neq 0$ we must have $\mpsol^\omega_q = 1$, in our SMWDS example this means that the arc capacity is $0$, since the indicator is $0$ if neither a vertex nor its neighbours are selected.  
 Thus we consider only the highlighted arcs in Figure \ref{fig:bdd1_cuts}, which we will denote from left to right $a_1$ and $a_2$. For both arcs we have $\pi_i - \pi_j = 1 > 0$, and we only have one indicator expression $x_0 + x_1+x_3$ on each arc, so we will ignore the indices $q \in \viol_a$ for ease of presentation. We can set $\hat{\beta}_{a_1} = \hat{\beta}_{a_2} = \pi_i - \pi_j =1$ and $\hat{\beta}_{aq} = 0$ for all other capacitated arcs $a$ and sets $\viol_a$. We have now obtained the cut:
\begin{equation} \label{eq:bdd1_cut_ex}
 \eta \geq 1 - 2(\xvar_{0} + \xvar_{1} + \xvar_{3} )
\end{equation}
which will be added to the master problem.
\end{example}
 
 
 \begin{figure}[h]
\begin{subfigure}[t]{0.5\textwidth}
	\centering
\hspace*{-1cm}		\begin{tikzpicture}[	main_node/.style={}, node distance = 1cm and 1cm,  > = stealth, % arrow head style
	%		shorten > = 0pt, % don't touch arrow head to node 
	]
	
	\node[main_node] (s) at  (-0.5,0) {$1$};
	
	\node[main_node] (l1n1) at (-2,-1.25) {$1$};
	\node[main_node] (l1n2) at  (1.5,-1.25) {$0$};
	
	\node[main_node] (l2n1) at (-3,-2.5) {$1$};
	\node[main_node] (l2n2) at (-1,-2.5) {$0$};
	\node[main_node] (l2n3) at (1,-2.5) {$0$};
	\node[main_node] (l2n4) at (3,-2.5) {$0$};
	
	\node[main_node] (l3n0) at (-5,-4) {$1$};
	\node[main_node] (l3n1) at (-3.25,-4) {$1$};
	\node[main_node] (l3n2) at (-1,-4) {$0$};
	\node[main_node](l3n3) at (0.5,-4) {$0$};
	\node[main_node] (l3n4) at (2,-4) {$0$};
	\node[main_node] (l3n5) at (3.5,-4) {$0$};
	
	
	\node[main_node] (l4n0) at (-5,-6) {$0$};
	\node[main_node] (l4n1) at (-3.5,-6) {$0$};
	\node[main_node](l4n2) at (0,-6) {$0$};
	\node[main_node] (l4n3) at (2.5,-6) {$0$};
	\node[main_node] (l4n4) at (3.75,-6) {$0$};
	
	\node[main_node](t) at (-.5,-8.5) {$0$};
	
	
	
	
	\draw[dashed, ->] (s) to (l1n1);
	\draw[->] (s) to (l1n2);
	
	\draw[dashed, ->] (l1n1) to  (l2n1);
	\draw[->] (l1n1) to (l2n2);
	\draw[dashed, ->] (l1n2) to []  (l2n3);
	\draw[->] (l1n2) to []  (l2n4);
	
	
	\draw[dashed, ->] (l2n1) to node[sloped, above, xshift=-0.1cm]{\scriptsize $x_0+x_1+x_2=1$} (l3n0);
	\draw[->] (l2n1) to (l3n1);
	\draw[dashed, ->] (l2n2) to (l3n2);
	\draw[->] (l2n2) to (l3n3);
	\draw[dashed, ->] (l2n3) to (l3n4);
	\draw[->] (l2n3) to (l3n3);
	\draw[dashed, ->] (l2n4) to (l3n5);
	\draw[->] (l2n4) to (l3n3);
	
	\draw[-, line width=4pt, color=CornflowerBlue] (l3n0) to (l4n0);
	\draw[dashed, ->] (l3n0) to [bend right=0] node[right, xshift =-0.25cm,rotate=0]{\scriptsize \begin{tabular}{l}
			$x_0+x_1$\\
			$+x_3=0$
	\end{tabular} }  (l4n0);
	\draw[->] (l3n0) to [bend right=8]  (l4n2);
	
	
	
	\draw[-, line width=4pt, color=CornflowerBlue] (l3n1) to [bend right=0]  (l4n2);
	\draw[dashed, ->] (l3n1) to [bend right=0] node[sloped, above, xshift=-.8cm, rotate=0]{\scriptsize  $x_0+x_1+x_3=0$}  (l4n2);
	\draw[->] (l3n1.south) to [bend right= 15]  (l4n2);
	
	\draw[dashed, ->] (l3n2.south) to  [bend left=10]  (l4n1.45);
	\draw[->] (l3n2) to (l4n2);
	
	\draw[dashed, ->] (l3n3) to [bend right=15]  (l4n2);
	\draw[->] (l3n3) to [bend left=15]  (l4n2);
	
	\draw[dashed, ->] (l3n4) to (l4n3);
	\draw[->] (l3n4) to (l4n2);
	\draw[dashed, ->] (l3n5) to (l4n4);
	\draw[->] (l3n5) to (l4n2);
	
	
	
	\draw[dashed, ->] (l4n0) to [bend right=0] node[sloped,below,rotate= 0 ]{\scriptsize
		\begin{tabular}{l}
			$x_1+x_2+x_3+x_4=1$,\\$x_0+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4=1$
	\end{tabular}}   (t);
	\draw[rounded corners=50pt,->] (l4n0.south) |- (t.west);
	
	
	\draw[dashed, ->] (l4n1.south) to [bend left=0] node[sloped,above, rotate=0 ]{\scriptsize
		\begin{tabular}{l}
			$x_0+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4=1$
	\end{tabular}}   (t.120);
	\draw[->] (l4n1.250) to [bend right=10]  (t.130);
	
	\draw[dashed, ->] (l4n2) to [bend right=15]  (t);
	\draw[->] (l4n2) to [bend left=15]  (t);
	
	\draw[dashed, ->] (l4n3) to [bend right=0] node[sloped, above, rotate= 0, xshift =0.5cm]{\scriptsize \begin{tabular}{l}
			$x_1+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4=1$
	\end{tabular} }   (t);
	\draw[->] (l4n3) to [bend left=20]  (t);
	
	\draw[dashed, ->] (l4n4.260) to [bend left=10] node[sloped, below, rotate=0]{\scriptsize $x_2+x_3+x_4=1$}   (t.east);
	
	\draw[->] (l4n4.280) to [bend left=400]  (t);
	
\end{tikzpicture}
 	\caption{ \bdd{2} subproblem solution for the SMWDS instance in Example \ref{ex:bdd1_cuts} at  \MP \ solution $\hat{\xvar} = [0,0,1,0,0]$. The nodes contain their dual values, and the highlighted arcs have capacity $0$. \label{fig:bdd1_cuts}}
\end{subfigure}
~
 \begin{subfigure}[t]{0.5\textwidth}
	\centering
\hspace*{1cm}		\begin{tikzpicture}[main_node/.style={},
		node distance = 1cm and 1cm,  > = stealth, % arrow head style
		shorten > = 1pt, % don't touch arrow head to node 
		]
		
		\node[main_node] (s) at  (0,0) {$1$};
		
		\node[main_node] (l1n1) at (-1.5,-1.5) {$1$};
		\node[main_node] (l1n2) at  (2,-1.5) {$0$};
		
		\node[main_node] (l2n1) at (-3,-3) {$1$};
		\node[main_node] (l2n2) at (3,-3) {$0$};
		
		
		\node[main_node] (l3n1) at (-3,-4.5) {$1$};
		\node[main_node](l3n2) at (0,-4.5) {$0$};
		\node[main_node] (l3n3) at (3,-4.5) {$1$};
		
		
		\node[main_node](l4n1) at (0,-6.5) {$0$};
		\node[main_node] (l4n2) at (3,-6.5) {$1$};
		
		
		\node[main_node](t) at (0,-8) {$0$};
		
		
		\draw[dashed, ->] (s) to (l1n1);
		\draw[->] (s) to node[sloped, above, rotate=0]{ \scriptsize$(1-\xvar_{0})=1$}  (l1n2);
		
		\draw[->] (l1n1) to node[sloped, above, rotate= 0]{ \scriptsize$(1-\xvar_{1})=1$}  (l2n2);
		\draw[dashed, ->] (l1n1) to (l2n1);
		
		\draw[dashed, ->] (l1n2) to [bend right=30]  (l2n2);
		\draw[->] (l1n2) to [bend left=30]  node[sloped, above, rotate= 0]{ \scriptsize$(1-\xvar_{1})=1$} (l2n2);
		
		
		
		\draw[-, line width=4.5pt, color=CornflowerBlue ] (l2n1) to (l3n1);
		\draw[->] (l2n1) to node[right, rotate= 0]{ \scriptsize$(1-\xvar_{2})=0$}  (l3n1);
		\draw[-, line width=4.5pt, color=CornflowerBlue ] (l2n2) to (l3n2);
		\draw[->] (l2n2) to node[above, sloped,rotate= 0]{ \scriptsize$(1-\xvar_{2})=0$}  (l3n2);
		\draw[dashed, ->] (l2n2) to (l3n3);
		
		
		\draw[->] (l3n1) to node[sloped, below, rotate= 0]{ \scriptsize$(1-\xvar_{3})=1$} (l4n1);
		\draw[dashed, ->] (l3n2) to [bend left=30]  (l4n1);
		\draw[->] (l3n2) to [bend right=30]  node[left, rotate= 0, yshift =0.4cm, xshift=0.3cm]{ \begin{tabular}{r}
				\scriptsize$(1-\xvar_{3})$\\	\scriptsize$=1$
		\end{tabular}}  (l4n1);
		\draw[dashed, ->] (l3n3) to  (l4n2);
		\draw[->] (l3n3) to node[sloped, below, rotate= 0]{ \scriptsize$(1-\xvar_{3})=1$}(l4n1);
		
		
		
		\draw[dashed, ->] (l4n1) to [bend left=30]  (t);
		\draw[->] (l4n1) to [bend right=30] node[left, rotate= 0, yshift =0.4cm]{ \scriptsize$(1-\xvar_{4})=1$}    (t);		
		\draw[->] (l4n2) to [] node[above, sloped, rotate= 0]{ \scriptsize$(1-\xvar_{4})=1$}   (t);
		
		
	\end{tikzpicture}
		\caption{\bdd{3} subproblem solution for the SMWDS instance in Example \ref{ex:bdd2_cuts} at \MP \ solution $\hat{\xvar} = [0,0,1,0,0]$. The nodes contain their dual values, and the highlighted 1-arcs have cost $0$.  \label{fig:bdd2_cuts}}
\end{subfigure}
\caption{BDD subproblem solutions for the SMWDS instance in Example \ref{ex:bdd1_cuts}  and in Example \ref{ex:bdd2_cuts}.}
 \end{figure}
 
 \begin{comment}
 \begin{figure}[h]
 	\centering
 		\begin{tikzpicture}[	main_node/.style={}, node distance = 1cm and 1cm,  > = stealth, % arrow head style
 		%		shorten > = 0pt, % don't touch arrow head to node 
 		]
 		
 		\node[main_node] (s) at  (-0.5,0) {$1$};
 		
 		\node[main_node] (l1n1) at (-2,-1.25) {$1$};
 		\node[main_node] (l1n2) at  (1.5,-1.25) {$0$};
 		
 		\node[main_node] (l2n1) at (-3,-2.5) {$1$};
 		\node[main_node] (l2n2) at (-1,-2.5) {$0$};
 		\node[main_node] (l2n3) at (1,-2.5) {$0$};
 		\node[main_node] (l2n4) at (3,-2.5) {$0$};
 		
 		\node[main_node] (l3n0) at (-5,-4) {$1$};
 		\node[main_node] (l3n1) at (-3.25,-4) {$1$};
 		\node[main_node] (l3n2) at (-1,-4) {$0$};
 		\node[main_node](l3n3) at (0.5,-4) {$0$};
 		\node[main_node] (l3n4) at (2,-4) {$0$};
 		\node[main_node] (l3n5) at (3.5,-4) {$0$};
 		
 		
 		\node[main_node] (l4n0) at (-5,-6) {$0$};
 		\node[main_node] (l4n1) at (-3.5,-6) {$0$};
 		\node[main_node](l4n2) at (0,-6) {$0$};
 		\node[main_node] (l4n3) at (2.5,-6) {$0$};
 		\node[main_node] (l4n4) at (3.75,-6) {$0$};
 		
 		\node[main_node](t) at (-.5,-8.5) {$0$};
 		
 		
 		
 		
 		\draw[dashed, ->] (s) to (l1n1);
 		\draw[->] (s) to (l1n2);
 		
 		\draw[dashed, ->] (l1n1) to  (l2n1);
 		\draw[->] (l1n1) to (l2n2);
 		\draw[dashed, ->] (l1n2) to []  (l2n3);
 		\draw[->] (l1n2) to []  (l2n4);
 		
 		
 		\draw[dashed, ->] (l2n1) to node[sloped, above, xshift=-0.1cm]{\scriptsize $x_0+x_1+x_2=1$} (l3n0);
 		\draw[->] (l2n1) to (l3n1);
 		\draw[dashed, ->] (l2n2) to (l3n2);
 		\draw[->] (l2n2) to (l3n3);
 		\draw[dashed, ->] (l2n3) to (l3n4);
 		\draw[->] (l2n3) to (l3n3);
 		\draw[dashed, ->] (l2n4) to (l3n5);
 		\draw[->] (l2n4) to (l3n3);
 		
 		\draw[-, line width=4pt, color=CornflowerBlue] (l3n0) to (l4n0);
 		\draw[dashed, ->] (l3n0) to [bend right=0] node[right, xshift =-0.25cm,rotate=0]{\scriptsize \begin{tabular}{l}
 				$x_0+x_1$\\
 				$+x_3=0$
 		\end{tabular} }  (l4n0);
 		\draw[->] (l3n0) to [bend right=8]  (l4n2);
 		
 		
 		
 		\draw[-, line width=4pt, color=CornflowerBlue] (l3n1) to [bend right=0]  (l4n2);
 		\draw[dashed, ->] (l3n1) to [bend right=0] node[sloped, above, xshift=-.8cm, rotate=0]{\scriptsize  $x_0+x_1+x_3=0$}  (l4n2);
 		\draw[->] (l3n1.south) to [bend right= 15]  (l4n2);
 		
 		\draw[dashed, ->] (l3n2.south) to  [bend left=10]  (l4n1.45);
 		\draw[->] (l3n2) to (l4n2);
 		
 		\draw[dashed, ->] (l3n3) to [bend right=15]  (l4n2);
 		\draw[->] (l3n3) to [bend left=15]  (l4n2);
 		
 		\draw[dashed, ->] (l3n4) to (l4n3);
 		\draw[->] (l3n4) to (l4n2);
 		\draw[dashed, ->] (l3n5) to (l4n4);
 		\draw[->] (l3n5) to (l4n2);
 		
 		
 		
 		\draw[dashed, ->] (l4n0) to [bend right=0] node[sloped,below,rotate= 0 ]{\scriptsize
 			\begin{tabular}{l}
 				$x_1+x_2+x_3+x_4=1$,\\$x_0+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4=1$
 		\end{tabular}}   (t);
 		\draw[rounded corners=50pt,->] (l4n0.south) |- (t.west);
 		
 		
 		\draw[dashed, ->] (l4n1.south) to [bend left=0] node[sloped,above, rotate=0 ]{\scriptsize
 			\begin{tabular}{l}
 				$x_0+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4=1$
 		\end{tabular}}   (t.120);
 		\draw[->] (l4n1.250) to [bend right=10]  (t.130);
 		
 		\draw[dashed, ->] (l4n2) to [bend right=15]  (t);
 		\draw[->] (l4n2) to [bend left=15]  (t);
 		
 		\draw[dashed, ->] (l4n3) to [bend right=0] node[sloped, above, rotate= 0, xshift =0.5cm]{\scriptsize \begin{tabular}{l}
 				$x_1+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4=1$
 		\end{tabular} }   (t);
 		\draw[->] (l4n3) to [bend left=20]  (t);
 		
 		\draw[dashed, ->] (l4n4.260) to [bend left=10] node[sloped, below, rotate=0]{\scriptsize $x_2+x_3+x_4=1$}   (t.east);
 		
 		\draw[->] (l4n4.280) to [bend left=400]  (t);
 		
 	\end{tikzpicture}
% 	\begin{tikzpicture}[main_node/.style={circle,fill=white!80,draw,inner sep=1pt, minimum size=35pt},
% 		line width=1.2pt, node distance = 1cm and 1cm,  > = stealth, % arrow head style
% 		shorten > = 1pt, % don't touch arrow head to node 
% 		]
% 		
% 		\node[main_node] (s) at  (0,0) {\small$1$};
% 		
% 		\node[main_node] (l1n1) at (-3,-1.5){\small$1$};
% 		\node[main_node] (l1n2) at  (3,-1.5) {\small$0$};
% 		
% 		\node[main_node] (l2n1) at (-5,-4){\small$1$};
% 		\node[main_node] (l2n2) at (-1,-4) {\small$0$};
% 		\node[main_node] (l2n3) at (1,-4)  {\small$0$};
% 		\node[main_node] (l2n4) at (5,-4)  {\small$0$};
% 		
% 		\node[main_node] (l3n0) at (-7,-6.5) {\small$1$};
% 		\node[main_node] (l3n1) at (-5,-6.5) {\small$1$};
% 		\node[main_node] (l3n2) at (-3,-6.5) {\small$0$};
% 		\node[main_node](l3n3) at (0,-6.5) {\small$0$};
% 		\node[main_node] (l3n4) at (3,-6.5) {\small$0$};
% 		\node[main_node] (l3n5) at (6,-6.5) {\small$0$};
% 		
% 		
% 		\node[main_node] (l4n0) at (-7,-9) {\small$0$};
% 		\node[main_node] (l4n1) at (-5,-9) {\small$0$};
% 		\node[main_node](l4n2) at (0,-9) {\small$0$};
% 		\node[main_node] (l4n3) at (4,-9) {\small$0$};
% 		\node[main_node] (l4n4) at (6,-9) {\small$0$};
% 		
% 		\node[main_node](t) at (0,-12) {\small$0$};
% 		
% 		
% 		\draw[dashed, ->] (s) to (l1n1);
% 		\draw[->] (s) to (l1n2);
% 		
% 		\draw[dashed, ->] (l1n1) to  (l2n1);
% 		\draw[->] (l1n1) to (l2n2);
% 		\draw[dashed, ->] (l1n2) to []  (l2n3);
% 		\draw[->] (l1n2) to []  (l2n4);
% 		
% 		
% 		\draw[dashed, ->] (l2n1) to node[above, rotate=50, yshift = .25cm]{\scriptsize $x_0+x_1+x_2 =1 $} (l3n0);
% 		\draw[->] (l2n1) to (l3n1);
% 		\draw[dashed, ->] (l2n2) to (l3n2);
% 		\draw[->] (l2n2) to (l3n3);
% 		\draw[dashed, ->] (l2n3) to (l3n4);
% 		\draw[->] (l2n3) to (l3n3);
% 		\draw[dashed, ->] (l2n4) to (l3n5);
% 		\draw[->] (l2n4) to (l3n3);
% 		
% 		 \draw[-, line width=4pt, color=CornflowerBlue] (l3n0) to [bend right=30]  (l4n0);
% 		\draw[dashed, ->] (l3n0) to [bend right=30] node[right, rotate=0]{\scriptsize  $x_0+x_1+x_3 =0$}  (l4n0);
%		\draw[->] (l3n0) to [bend right=5]  (l4n2);
% 		 
% 		 \draw[-, line width=4pt, color=CornflowerBlue] (l3n1) to [bend right=30]  (l4n2);
% 		\draw[dashed, ->] (l3n1) to [bend right=30] node[below, rotate= -30]{\scriptsize  $x_0+x_1+x_3 =0 $}  (l4n2);
% 		\draw[->] (l3n1) to [bend left= 5]  (l4n2);
% 		
% 		\draw[dashed, ->] (l3n2) to (l4n1);
% 		\draw[->] (l3n2) to (l4n2);
% 		
% 		\draw[dashed, ->] (l3n3) to [bend right=30]  (l4n2);
% 		\draw[->] (l3n3) to [bend left=30]  (l4n2);
% 		
% 		\draw[dashed, ->] (l3n4) to (l4n3);
% 		\draw[->] (l3n4) to (l4n2);
% 		\draw[dashed, ->] (l3n5) to (l4n4);
% 		\draw[->] (l3n5) to (l4n2);
% 		
% 		
% 		
% 		\draw[dashed, ->] (l4n0) to [bend right=40] node[below,rotate= -30 ]{\scriptsize
% 			\begin{tabular}{l}
% 				$x_1+x_2+x_3+x_4 =1$,\\$x_0+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4 =1$
% 		\end{tabular}}   (t);
% 		\draw[->] (l4n0) to [bend left=0]  (t);
% 		
% 		
% 		\draw[dashed, ->] (l4n1) to [bend right=20] node[below,rotate= -30 ]{\scriptsize
% 			\begin{tabular}{l}
% 				$x_0+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4=1$
% 		\end{tabular}}   (t);
% 		\draw[->] (l4n1) to [bend left=20]  (t);
% 		
% 		\draw[dashed, ->] (l4n2) to [bend right=30]  (t);
% 		\draw[->] (l4n2) to [bend left=30]  (t);
% 		
% 		\draw[dashed, ->] (l4n3) to [bend right=20] node[above, rotate= 30, xshift =0.5cm]{\scriptsize \begin{tabular}{l}
% 				$x_1+x_2+x_3+x_4=1$,\\ $x_2+x_3+x_4=1$
% 		\end{tabular} }   (t);
% 		\draw[->] (l4n3) to [bend left=45]  (t);
% 		
% 		\draw[dashed, ->] (l4n4) to [bend left=45] node[below, rotate=30]{\scriptsize $x_2+x_3+x_4=1$}   (t);
% 		\draw[->] (l4n4) to [bend right=0]  (t);
% 		
% 	\end{tikzpicture}
% 	
 	\caption{ \bdd{2} subproblem solution for the SMWDS instance in Example \ref{ex:bdd1_cuts} at  \MP \ solution $\hat{\xvar} = [0,0,1,0,0]$. The nodes contain their dual values, and the highlighted arcs have capacity $0$. \label{fig:bdd1_cuts}}
 \end{figure}
\end{comment}
For a fixed scenario $\omega$ the Benders cuts that come those that come from \bdd{3} are:
 \begin{equation} \label{eq:bdd2_cuts}
\eta_\omega \geq \hat{\pi}_\rootnode   - \sum_{a  \in \onearcs} \hat{z}_a\indvar_{\map(a)} .
 \end{equation} 
The procedure to obtain the duals for the \bdd{3} subproblems is very similar to that for  the \bdd{2} subproblems. For a scenario BDD $\BDD^\omega$ and master problem solution $\hat{\indvar}$, we calculate the dual solutions using a bottom-up shortest-path algorithm, starting at the terminal node which has $\pi_\term = 0$. For each subsequent node $i$, $\pi_i$ is the length of the shortest $i$-$\term$ path. 
As seen in \eqref{form:BDD2_dual2}, the $z_a$ variables correspond only to arcs in $\onearcs$. By constraints \eqref{eq:D2_pizUB} and $\eqref{eq:D2_zbd}$, if $\pi_i - \pi_j - \costtwo{\map(a)} \leq 0 $, 
we can set $z_a = 0$. Otherwise, we set $ z_a = \pi_i - \pi_j -\costtwo{\map(a)} $. In this way, $z_a + \costtwo{\map(a)} $ can be seen as the change in path length between $i$ and $j$.


 \begin{example} \label{ex:bdd2_cuts}
	We will compute a cut at master problem solution $\hat{\xvar} = [0,0,1,0,0]$ for the BDD built in Example \ref{ex:bdd2}. As seen by the highlighted arcs in Figure \ref{fig:bdd2_cuts}, at this solution we have two arcs in $\onearcs$ that now have cost $0$. Using the parametrized arc costs we compute the shortest path dual values $\pi$ which can be seen inside the nodes in Figure  \ref{fig:bdd2_cuts}. To find the values of the $z_a$ variables, we will compute $\pi_i -\pi_j$ for all $a = (i,j) \in \onearcs$ and set $z_a$ accordingly.  These values can be seen next to the arcs in Figure \ref{fig:bdd2_cuts}. 
	Taking $\xvar_{\map(a)}$ as the indicator we have now obtained the cut:
	\begin{equation} \label{eq:bdd2_cut_ex}
	\eta \geq 1 - (\xvar_{0} + \xvar_{1} + \xvar_{3} + 2 \xvar_{4}).
	\end{equation}
	We remark that this cut differs from the cut found in Example \ref{ex:bdd1_cuts} despite being derived for the same subproblem instance at the same master problem solution.
\end{example}
\begin{comment}
	\begin{figure}[h]
		\centering
			\begin{tikzpicture}[main_node/.style={},
			node distance = 1cm and 1cm,  > = stealth, % arrow head style
			shorten > = 1pt, % don't touch arrow head to node 
			]
			
			\node[main_node] (s) at  (0,0) {$1$};
			
			\node[main_node] (l1n1) at (-1.5,-1.5) {$1$};
			\node[main_node] (l1n2) at  (2,-1.5) {$0$};
			
			\node[main_node] (l2n1) at (-3,-3) {$1$};
			\node[main_node] (l2n2) at (3,-3) {$0$};
			
			
			\node[main_node] (l3n1) at (-3,-4.5) {$1$};
			\node[main_node](l3n2) at (0,-4.5) {$0$};
			\node[main_node] (l3n3) at (3,-4.5) {$1$};
			
			
			\node[main_node](l4n1) at (0,-6.5) {$0$};
			\node[main_node] (l4n2) at (3,-6.5) {$1$};
			
			
			\node[main_node](t) at (0,-8) {$0$};
			
			
			\draw[dashed, ->] (s) to (l1n1);
			\draw[->] (s) to node[sloped, above, rotate=0]{ \scriptsize$(1-\xvar_{0})=1$}  (l1n2);
			
			\draw[->] (l1n1) to node[sloped, above, rotate= 0]{ \scriptsize$(1-\xvar_{1})=1$}  (l2n2);
			\draw[dashed, ->] (l1n1) to (l2n1);
			
			\draw[dashed, ->] (l1n2) to [bend right=30]  (l2n2);
			\draw[->] (l1n2) to [bend left=30]  node[sloped, above, rotate= 0]{ \scriptsize$(1-\xvar_{1})=1$} (l2n2);
			
			
			
			\draw[-, line width=4.5pt, color=CornflowerBlue ] (l2n1) to (l3n1);
			\draw[->] (l2n1) to node[right, rotate= 0]{ \scriptsize$(1-\xvar_{2})=0$}  (l3n1);
			\draw[-, line width=4.5pt, color=CornflowerBlue ] (l2n2) to (l3n2);
			\draw[->] (l2n2) to node[above, sloped,rotate= 0]{ \scriptsize$(1-\xvar_{2})=0$}  (l3n2);
			\draw[dashed, ->] (l2n2) to (l3n3);
			
			
			\draw[->] (l3n1) to node[sloped, below, rotate= 0]{ \scriptsize$(1-\xvar_{3})=1$} (l4n1);
			\draw[dashed, ->] (l3n2) to [bend left=30]  (l4n1);
			\draw[->] (l3n2) to [bend right=30]  node[left, rotate= 0, yshift =0.4cm, xshift=0.3cm]{ \begin{tabular}{r}
					\scriptsize$(1-\xvar_{3})$\\	\scriptsize$=1$
				\end{tabular}}  (l4n1);
			\draw[dashed, ->] (l3n3) to  (l4n2);
			\draw[->] (l3n3) to node[sloped, below, rotate= 0]{ \scriptsize$(1-\xvar_{3})=1$}(l4n1);
			
			
			
			\draw[dashed, ->] (l4n1) to [bend left=30]  (t);
			\draw[->] (l4n1) to [bend right=30] node[left, rotate= 0, yshift =0.4cm]{ \scriptsize$(1-\xvar_{4})=1$}    (t);		
			\draw[->] (l4n2) to [] node[above, sloped, rotate= 0]{ \scriptsize$(1-\xvar_{4})=1$}   (t);
			
			
		\end{tikzpicture}
		
		\begin{tikzpicture}[main_node/.style={circle,fill=white!80,draw,inner sep=1pt, minimum size=35pt},
			line width=1.2pt, node distance = 1cm and 1cm,  > = stealth, % arrow head style
			shorten > = 1pt, % don't touch arrow head to node 
			]
			
			\node[main_node] (s) at  (0,0) {\small$1$};
			
			\node[main_node] (l1n1) at (-4,-1.5) {\small$1$};
			\node[main_node] (l1n2) at  (4,-1.5) {\small$0$};
			
			\node[main_node] (l2n1) at (-4,-4){\small$1$};
			\node[main_node] (l2n2) at (4,-4){\small$0$};
			
			
			\node[main_node] (l3n1) at (-4,-6.5) {\small$1$};
			\node[main_node](l3n2) at (0,-6.5) {\small$0$};
			\node[main_node] (l3n3) at (4,-6.5){\small$1$};
			
			
			\node[main_node](l4n1) at (0,-9){\small$0$};
			\node[main_node] (l4n2) at (4,-9) {\small$1$};
			
			
			\node[main_node](t) at (0,-12){\small$0$};
			
			
			\draw[dashed, ->] (s) to (l1n1);
			\draw[->, white] (s) to node[below, rotate=-20] {\scriptsize\cblue$1$}  (l1n2);
			\draw[->] (s) to node[above, rotate=-20]{ \scriptsize$(1-\xvar_{0}) =1$}  (l1n2);
			
			\draw[->, white] (l1n1) to node[below, rotate=-20] {\scriptsize\cblue$1$}  (l2n2);
			\draw[->] (l1n1) to node[above, rotate= -20]{ \scriptsize$(1-\xvar_{1})=1$}  (l2n2);
			\draw[dashed, ->] (l1n1) to (l2n1);
			
			\draw[dashed, ->] (l1n2) to [bend right=30]  (l2n2);
			\draw[->, white]  (l1n2) to  [bend left=30] node[left, rotate=0] {\scriptsize\cblue$0$}  (l2n2);
			\draw[->] (l1n2) to [bend left=30]  node[right, rotate= 0]{ \scriptsize$(1-\xvar_{1})=1$} (l2n2);
		
			\draw[-, line width=4.5pt, color=CornflowerBlue ] (l2n1) to node[left, rotate= 0]{\scriptsize\cblue$0$} (l3n1);
			\draw[->] (l2n1) to node[right, rotate= 0]{ \scriptsize$(1-\xvar_{2}) =0$}  (l3n1);
		
			\draw[-, line width=4.5pt, color=CornflowerBlue ]  (l2n2) to node[below, rotate= 30] {\scriptsize\cblue$0$}  (l3n2);
			\draw[->] (l2n2) to node[above, rotate= 30]{ \scriptsize$(1-\xvar_{2})=0 $}  (l3n2);
			\draw[dashed, ->] (l2n2) to (l3n3);
			
			
			\draw[->, white]  (l3n1) to node[above, rotate= -30] {\scriptsize\cblue$1$}   (l4n1);
			\draw[->] (l3n1) to node[below, rotate= -30]{ \scriptsize$(1-\xvar_{3})=1$} (l4n1);
			\draw[dashed, ->] (l3n2) to [bend left=30]  (l4n1);
			\draw[->, white]  (l3n2) to [bend right=30]  node[right, rotate= 0, yshift =0.2cm] {\scriptsize\cblue$0$}   (l4n1);
			\draw[->] (l3n2) to [bend right=30]  node[left, rotate= 0, yshift =0.4cm]{ \scriptsize$(1-\xvar_{3})=1$}  (l4n1);
			\draw[dashed, ->] (l3n3) to  (l4n2);
			\draw[->, white]  (l3n3) to node[above, rotate= 30] {\scriptsize\cblue$1$}   (l4n1);
			\draw[->] (l3n3) to node[below, rotate= 30]{ \scriptsize$(1-\xvar_{3})=1$}(l4n1);
			
			
			
			\draw[dashed, ->] (l4n1) to [bend left=30]  (t);
			\draw[->, white]  (l4n1) to [bend right=30] node[right, rotate= 0, yshift =0cm]{\scriptsize\cblue$0$}   (t);
			\draw[->] (l4n1) to [bend right=30] node[left, rotate= 0, yshift =0cm]{ \scriptsize$(1-\xvar_{4})=1$}    (t);		
			\draw[->, white] (l4n2) to [] node[above, rotate= 30] {\scriptsize\cblue$1$}   (t);
			\draw[->] (l4n2) to [] node[below, rotate= 30]{ \scriptsize$(1-\xvar_{4})=1$}   (t);
			
			
		\end{tikzpicture}

		\caption{\bdd{3} subproblem solution for the SMWDS instance in Example \ref{ex:bdd1_cuts} at \MP \ solution $\hat{\xvar} = [0,0,1,0,0]$. The nodes contain their dual values, and the highlighted 1-arcs have cost $0$.  \label{fig:bdd2_cuts}}
	\end{figure}
\end{comment}


We remark that we are able to apply the cut strengthening strategies proposed by Lozano and Smith \cite{lozano2018bdd} to both cuts  \eqref{eq:bdd1_cuts} and \eqref{eq:bdd2_cuts}. The first strategy relies on partitioning $\arcs^\omega$ into disjoint sets of arcs and selecting the maximal value of $\hat{\beta}_{aq}$ or $\hat{z}_a$ from each set to appear in the cut.
First remark that the BDD arc layers, $\arclayer{i}$ for all $i \in \{1, \hdots, m_1\}$ are disjoint and partition $\arcs^\omega$. In \bdd{2}, for each $i \in \{1, \hdots, m_1\}$, let $\kappa^i$ be the arc for which $\hat{\beta}_{\kappa^i q} = \arg \max_{a \in \arclayer{i}}\{\hat{\beta}_{aq} : q \in \viol_a\}$. 
Similarly, in \bdd{3}, define $\kappa^i$ for $i \in \{1, \hdots, m_1\}$ as the arc for which $\hat{z}_{\kappa^i} = \arg \max_{a \in \arclayer{i}}\{\hat{z}_{a}\}$.
For both types of BDDs, let $\Gamma = \cup_{i \in \{1, \hdots, m_1\}} \{\kappa^i\}$.
%
%
%
%For each $\arclayer{i}$ we will use only the maximal value of $\beta_{aq}$ or $z_a$ in the cut, as this is necessarily 
%
%

%	We use the layers $\arclayer{i}$ for all $i \in \{1, \hdots, n_3\}$ as the partition and let $\Gamma = \cup_{i \in \{1, \hdots, m_1\}} \arg \max_{a \in \arclayer{i}}\{\hat{\beta}_{aq} : q \in \viol_a\}$  for \bdd{2} or $\Gamma = \cup_{i \in \{1, \hdots, m_1\}} \arg \max_{j \in \arclayer{i}}\{\hat{z}_j\}$ for \bdd{3}. 
Then the cut
\begin{equation}  \label{eq:bdd1_cut_stren}
	\eta_\omega \geq \hat{\pi}_\rootnode - \sum_{a  \in \Gamma} \sum_{i \in \viol_a} \hat{\beta}_{aq}(1 - \indvar_i)
\end{equation} 
 is at least as good as \eqref{eq:bdd1_cuts} and the cut
  \begin{equation} \label{eq:bdd2_cut_stren}
 	\eta_\omega \geq \hat{\pi}_\rootnode   - \sum_{a  \in \Gamma} \hat{z}_a\indvar_{\map(a)} .
 \end{equation} 
  is at least as good as \eqref{eq:bdd2_cuts}. Henceforth we assume the use of these strengthened cuts for \bdd{2} and \bdd{3} unless otherwise stated. 
  
  The second strengthening strategy solves a secondary optimization problem to help compute lower bounds on the second-stage objective function which are then used to strengthen the cut. We refer the reader to Lozano and Smith \cite{lozano2018bdd} for further details on the cut strengthening strategies.
  
  \begin{example}\label{ex:str_cuts}
 For the scenario graph in Figure \ref{fig:smwds_graph}, the strengthened version of the cut \eqref{eq:bdd1_cut_ex}  is 
 \begin{equation} \label{eq:bdd1_cut_ex_str}
 	\eta \geq 1 - (\xvar_{0} + \xvar_{1} + \xvar_{3} )
 \end{equation}
and  the strengthened version of the cut \eqref{eq:bdd2_cut_ex} is
 	\begin{equation} \label{eq:bdd2_cut_ex_str}
 	\eta \geq 1 - (\xvar_{0} + \xvar_{1} + \xvar_{3} +  \xvar_{4}).
 \end{equation}
 
 
  \end{example}

